TokenSynth: A Token-based Neural Synthesizer for Instrument Cloning and Text-to-Instrument

Recent advancements in neural audio codecs have enabled the use of tokenized audio representations in various audio generation tasks, such as text-to-speech, text-to-audio, and text-to-music generation. Leveraging this approach, we propose TokenSynth, a novel neural synthesizer that utilizes a decoder-only transformer to generate desired audio tokens from MIDI tokens and CLAP (Contrastive Language-Audio Pretraining) embedding, which has timbre-related information. Our model is capable of performing instrument cloning, text-to-instrument synthesis, and text-guided timbre manipulation without any fine-tuning. This flexibility enables diverse sound design and intuitive timbre control. We evaluated the quality of the synthesized audio, the timbral similarity between synthesized and target audio/text, and synthesis accuracy (i.e., how accurately it follows the input MIDI) using objective measures. TokenSynth demonstrates the potential of leveraging advanced neural audio codecs and transformers to create powerful and versatile neural synthesizers. The source code, model weights, and audio demos are available at: https://github.com/KyungsuKim42/tokensynth

==> musicography.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{musicography}[2023/09/08
  Symbols for music writing with pdflatex]

% Copyright 2023 Andrew A. Cashner, andrewacashner@gmail.com

% This work may be distributed and/or modified under the 
% conditions of the LaTeX Project Public License, either
% version 1.3 of this license or (at your option) any 
% later version.
% The latest version of this license is in 
%    http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions
% of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% The Current Maintainer of this work is Andrew A. Cashner.
% This work consists of the package file musicography.sty
% and the documentation file musicography.tex.

% CHANGE LOG
% 2023-09-08 - Improved time signatures, figured bass, documentation
%               + Documentation reorganized, clarified, corrected
%               + Customizable font commands used throughout:
%                 \musAccidentalFont, \musNumFont, \musFigSize, and
%                 \musFigFont 
%               + \musStack now takes an optional last argument to specify
%                 alignment
%               + \musMeter now takes an optional font argument, and has a
%                 smaller vertical gap between numerals. It is now scaled
%                 to fit within the line.
%               + Spacing commands in \musSymbolMeter are simplified
%               + \meterThreeTwo now uses \musMeter for the numbers, shifted
%                 slightly to align with the meter symbol
%               + \meterCZ now pulls in a cursive Z symbol from the EB
%                 Garamond font (installed by default in TeXLive)
%               + \musFig now includes configurable \musFigSize and
%                 \musFigFont switches, and a first optional argument with
%                 alignment specifier
%               + New commands for scale degress (\musDegree) and pitches with
%                 Helmholtz octave (\musPitch)
%               + For testing or extension, add command to display a list of
%                 symbols by number in a given font
%
% 2020-01-29 - Reduced stack gap for \musFig
% 2019-11-24 - Fix problem with \MeterCThreeTwo where numerals were being
%               printed next to each other instead of stacked.
% 2019-05-28 - Fix issue #1:
%               + Correct notehead symbol for values < quarter note
%                 (was hollow, should be filled)
%               + Add 32nd and 64th notes regular and dotted
%               + \musSymbol now inside an \mbox to fix alignment problems
%            - New features (some requested in issue #1)
%               + Add medieval perfect meter
%               + Add aliases for fusa (= corchea = eighth note)
%               + Replace musStack implementation with stackengine:
%                 Now takes any number of space-separated arguments to stack
%                 numerals, allowing for full figured-bass notation
% 2018-05-21 Override semantic-markup's \fl, \sh, \na commands if it is loaded
% 2017-10-31 Corrected glyph for \musHalf and documented
%              \musMeter and \musFigures
% 2017-08-29 First version on CTAN
% 2017-04-12 Created

% FONT SIZES

% Package option 'bigger'
%
% The package uses three sizes of music fonts;  the 'bigger' option increases
%  all three.
\newif\ifLargeFont
\LargeFontfalse
\DeclareOption{bigger}{\LargeFonttrue}
\ProcessOptions\relax

\ifLargeFont
    \newfont{\musFont}{musix13}
    \newfont{\musFontBig}{musix16}
    \newfont{\musFontLarge}{musix20}
\else
    \newfont{\musFont}{musix11}
    \newfont{\musFontBig}{musix13}
    \newfont{\musFontLarge}{musix16}
\fi

% BASIC COMMANDS

% Print a music symbol from the \musFont, specifying space before, after, and
% baseline adjustment
%  #1 optional font command (default: \musFont)
%  #2 kern before    
%  #3 raisebox value 
%  #4 kern after     
%  #5 symbol code (e.g., \symbol{4}) 
\NewDocumentCommand{\musSymbol}{ O{\musFont} m m m m }{%
    \mbox{#1\kern#2\raisebox{#3}{#5}\kern#4}%
}

% ACCIDENTALS

% Larger relative font for accidentals (can be modified)
\NewDocumentCommand{\musAccidentalFont}{}{\musFontLarge}

% Any accidental
%  #1 symbol command for accidental
\NewDocumentCommand{\musAccidental}{ m }{%
    \musSymbol[\musAccidentalFont]{0.1em}{0.5ex}{-0.1pt}{#1}%
}

% Specific accidentals
\NewDocumentCommand{\musFlat}       {}{\musAccidental{\symbol{90}}}
\NewDocumentCommand{\musDoubleFlat} {}{\musAccidental{\symbol{91}}}
\NewDocumentCommand{\musSharp}      {}{\musAccidental{\symbol{92}}}
\NewDocumentCommand{\musDoubleSharp}{}{\musAccidental{\symbol{93}}}
\NewDocumentCommand{\musNatural}    {}{\musAccidental{\symbol{94}}}

% Shorthand accidental commands
%
% These commands are defined differently in the semantic-markup package,
% so LaTeX will use musicography commands instead
\@ifpackageloaded{semantic-markup}{%
    \RenewDocumentCommand{\fl}{}{\musFlat}
    \RenewDocumentCommand{\sh}{}{\musSharp}
    \RenewDocumentCommand{\na}{}{\musNatural}
}{%
    \NewDocumentCommand{\fl}{}{\musFlat}
    \NewDocumentCommand{\sh}{}{\musSharp}
    \NewDocumentCommand{\na}{}{\musNatural}
}

% MUSIC NOTES

% Just the stem
\NewDocumentCommand{\musStem}{}{%
    \musSymbol{0.955em}{0.55ex}{0pt}{\symbol{16}}%
}

% Just the (augmentation) dot 
\NewDocumentCommand{\musDot}{}{%
    \musSymbol{-0.2em}{-0.5ex}{0.7em}{\symbol{24}}%
}

% Notehead plus stem (composite music symbol)
%  #1 Symbol musSymbol command for notehead
\NewDocumentCommand{\musStemmedNote}{ m }{%
    \musSymbol{0.05em}{0.5ex}{0.2em}{#1\musStem}%
}

% Stemmed note plus flag
%  #1 symbol command for base note
%  #2 symbol command for flag
\NewDocumentCommand{\musFlaggedNote}{ m m }{%
    \musSymbol{0.05em}{0.5ex}{0pt}{#1\musStem}%
    \musSymbol{0pt}{0pt}{0.9em}{#2}%
}

% Dotted note
%  #1 \musSymbol command for note to be dotted
\NewDocumentCommand{\musDottedNote}{ m }{#1\musDot}


% Notes of different rhythmic values
\NewDocumentCommand{\musBreve}{}{%
    \musSymbol{0.05em}{0.5ex}{1.35em}{\symbol{32}}%
}
\NewDocumentCommand{\musWhole}{}{%
    \musSymbol{0.05em}{0.5ex}{1.35em}{\symbol{9}}%
}
\NewDocumentCommand{\musHalf}{}{%
    \musStemmedNote{\symbol{8}}%
}
\NewDocumentCommand{\musQuarter}{}{%
    \musStemmedNote{\symbol{7}}%
}
\NewDocumentCommand{\musEighth}{}{%
    \musFlaggedNote{\symbol{7}}{\symbol{40}}%
}
\NewDocumentCommand{\musSixteenth}{}{%
    \musFlaggedNote{\symbol{7}}{\symbol{41}}%
}
\NewDocumentCommand{\musThirtySecond}{}{%
    \musFlaggedNote{\symbol{7}}{\symbol{42}}%
}
\NewDocumentCommand{\musSixtyFourth}{}{%
    \musFlaggedNote{\symbol{7}}{\symbol{43}}%
}

% Dotted rhythmic values
\NewDocumentCommand{\musWholeDotted}{}{%
    \musDottedNote{\musWhole}%
}
\NewDocumentCommand{\musHalfDotted}{}{%
    \musDottedNote{\musHalf}%
}
\NewDocumentCommand{\musQuarterDotted}{}{%
    \musDottedNote{\musQuarter}%
}
\NewDocumentCommand{\musEighthDotted}{}{%
    \musDottedNote{\musEighth}%
}
\NewDocumentCommand{\musSixteenthDotted}{}{%
    \musDottedNote{\musSixteenth}%
}
\NewDocumentCommand{\musThirtySecondDotted}{}{%
    \musDottedNote{\musThirtySecond}%
}
\NewDocumentCommand{\musSixtyFourthDotted}{}{%
    \musDottedNote{\musSixtyFourth}%
}

% Aliases for older note names
\NewDocumentCommand{\musSemibreve}         {}{\musWhole}
\NewDocumentCommand{\musMinim}             {}{\musHalf}
\NewDocumentCommand{\musSemiminim}         {}{\musQuarter}
\NewDocumentCommand{\musCorchea}           {}{\musEighth}
\NewDocumentCommand{\musFusa}              {}{\musEighth}
\NewDocumentCommand{\musSemibreveDotted}   {}{\musWholeDotted}
\NewDocumentCommand{\musMinimDotted}       {}{\musHalfDotted}
\NewDocumentCommand{\musSeminiminimDotted} {}{\musQuarterDotted}
\NewDocumentCommand{\musCorcheaDotted}     {}{\musEighthDotted}
\NewDocumentCommand{\musFusaDotted}        {}{\musEighthDotted}


% STACKED NUMERALS (for figured bass, time signatures)

\RequirePackage{stackengine}

% Only a minimal vertical gap between stacked elements
\setstackgap{S}{1pt}

% Specify the font for numbers in \musStack. For time signatures I think bold
% numbers look better in most fonts, but you could redefine it, for example,
% to use lining figures, math mode, sans-serif, etc.
%
% Example: To get lining figures when using the ebgaramond package:
% \renewcommand{\musNumFont}{\liningnums}
%
% The command is employed in a way that both font switches and commands with
% arguments will work (e.g., {\bfseries\liningnums}), but take care when
% combining multiple elements.
\NewDocumentCommand{\musNumFont}{}{\bfseries}

% Command to stack numerals for metrical symbols or figured bass
% Takes any number of space-separated arguments and stacks them vertically
% 
% #1 (optional) Font command (\musNumFont by default)
% #2 Series of space-separated arguments to be stacked, e.g., {\fl6 5}
% #3 (optional) Alignment specifier for \Shortstack (l, c, or r); default is c
%    for centering
\NewDocumentCommand{\musStack}{ O{\musNumFont} m O{c} }{%
    {#1{\Shortstack[#3]{#2}}}%
}

% METER and TIME SIGNATURES

\RequirePackage{graphicx} % for resizebox

% Numeric meter signatures (e.g., 3/4)
%  #1 (optional) font command (\musNumFont by default)
%  #1 number on top
%  #2 number on bottom
%
% In a pinch you can issue a font command directly in the optional first
% argument, but it would be better to redefine \musNumFont.
%
% These are now scaled to the current line height and centered.
\NewDocumentCommand{\musMeter}{ O{\musNumFont} m m }{%
    \resizebox{!}{\ht\strutbox}{%
        \musStack[#1]{#2 #3}%
    }\kern0.05em
}

% Meter symbols
%  #1 symbol code for meter sign
\NewDocumentCommand{\musSymbolMeter}{ m }{%
    \smash{\kern-1pt\musFontBig\raisebox{1.1ex}{#1}\kern0.3em}%
}

% Meter symbol plus numerals
\NewDocumentCommand{\meterPlus}{ m m }{#1\kern-0.7pt#2}

% Meter signatures with a C or cut C symbol
% Just the symbols
\NewDocumentCommand{\meterC}{}{%
    \musSymbolMeter{\symbol{83}}%
}
\NewDocumentCommand{\meterCutC}{}{%
    \musSymbolMeter{\symbol{82}}%
}

% Ternary meters used in 16th--18th c. music
% Just the numbers: 3
\NewDocumentCommand{\meterThree}{}{%
    {\musNumFont{3}}%
}

% 3/2
\NewDocumentCommand{\meterThreeTwo}{}{%
    \raisebox{-0.26ex}{\musMeter{3}{2}}%
}

% Combining symbols and numbers
% Meter that combines \meterC with numerals (e.g., C3 C3/2)
\NewDocumentCommand{\meterCplus}{ m }{\meterPlus{\meterC}{#1}}

% Meter that combines \meterCutC with numerals (e.g., C3 C3/2)
\NewDocumentCommand{\meterCutCplus}{ m }{\meterPlus{\meterCutC}{#1}}

% Proportions of cut C
\NewDocumentCommand{\meterCutCThree}{}{%
    \meterCutCplus{\meterThree}%
}
\NewDocumentCommand{\meterCutCThreeTwo}{}{%
    \meterCutCplus{\meterThreeTwo}%
}

% Proportions of C
\NewDocumentCommand{\meterCThree}{}{%
    \meterCplus{\meterThree}%
}
\NewDocumentCommand{\meterCThreeTwo}{}{%
    \meterCplus{\meterThreeTwo}%
}

% CZ meter: Ternary meter used in 17th-century Spanish music
%
% A cursive Z to match the C meter symbol, as notated in Spanish manuscripts
%
% Pull in symbol from EB Garamond font; could be redefined
\NewDocumentCommand{\meterZfont}{}{%
    \fontfamily{EBGaramond-LF}\selectfont
}

% The symbol
\NewDocumentCommand{\meterZsymbol}{}{%
    {\meterZfont\Large\itshape z}%
}

% CZ meter
\NewDocumentCommand{\meterCZ}{}{%
    \meterCplus{\meterZsymbol}%
}

% Perfect meter in medieval music
\NewDocumentCommand{\meterO}{}{%
    $\bigcirc$
}


% FIGURED BASS

% Definable font command to be used with figured bass; consider matching
% \musNumFont (e.g., with lining numerals)
\NewDocumentCommand{\musFigFont}{}{}

% Size adjustment for figured bass: smaller font for numerals, reduce sizes of
% music symbols (\tiny might make it fit better within the line height)
\NewDocumentCommand{\musFigSize}{}{%
    \scriptsize
    \RenewDocumentCommand{\musAccidentalFont}{}{\musFont}%
}

% Figured bass is typeset a \musStack using \musFigFont, right-aligned to
% allow for accidentals preceding numerals
%  #1 (optional) Alignment specifier: l, c, r (default: r)
%  #2 space-delimited list of arguments to stack, in top-down order
% 
% Example: \musFig{\fl6 4} or \musFig{\sh5 4 2}
%
% Note that the command applies first \musFigSize, then \musFigFont inside the
% stack.
\NewDocumentCommand{\musFig}{ O{r} m }{%
    {\musFigSize\musStack[\musFigFont]{#2}[#1]}%
}

% Placeholder for no figure, to maintain alignment
%  #1 (optional) width of blank space (Default: numeral 5)
%
% Example: \musFig{6 4}--\musFig{5 \noFig}
\NewDocumentCommand{\noFig}{ O{5} }{%
    \hphantom{#1}%
}

% MISCELLANEOUS SYMBOLS and NOTATIONS

% Segno (repeat marker)
\NewDocumentCommand{\musSegno}{}{%
    \musSymbol{0.55em}{-0.4ex}{1.5em}{\symbol{86}}%
}

% Scale degrees
% #1 Numeral (offset from tonic)
\NewDocumentCommand{\musDegree}{ m }{$\hat{#1}$}

% Pitch with Helmholtz octave number (e.g., A4 = A440Hz)
% #1 Pitch-class name (A-G)
% #2 Octave number
\NewDocumentCommand{\musPitch}{ m m }{#1\textsubscript{#2}}

% Recommended: Use my 'octave' package for more options, including
% traditional, non-Helmholtz notation

% AUXILIARY COMMANDS

% Print a list of symbols for documentation, debugging, or extension
% E.g., \symbolList{\musFont}{256} to see all useable symbols in MusiXTeX font

\RequirePackage{setspace} % for symbol list spacing

\ExplSyntaxOn
% Single entry in the symbol list: Number + corresponding symbol
%  #1 font command
%  #2 symbol number
\cs_new:Nn \aac_symbolEntry:nn
{
    \makebox[4em]{#2\quad{#1\symbol{#2}}}\ %
}

% Loop through all the symbols in given font up to given max
%  #1 font command
%  #2 max symbol number
\cs_new:Nn \aac_symbolLoop:nn
{
    \int_step_inline:nnn {0} {#2 - 1}
    {
        \aac_symbolEntry:nn {#1} {##1}
    }
}


% The whole symbol list up to a given max, typeset in a big double-spaced
% block
%  #1 font command
%  #2 max symbol number
\NewDocumentCommand{\symbolList}{ m m }{\par
    \begin{doublespace}
        \noindent\aac_symbolLoop:nn {#1} {#2}
    \end{doublespace}
}
\ExplSyntaxOff

% Print a list of symbols in the MusiXTeX font
\NewDocumentCommand{\musixSymbolList}{}{\symbolList{\musFont}{128}}

\endinput
